Automated Multi-Label Classification based on ML-Plan

Automated machine learning (AutoML) has received increasing attention in the recent past. While the main tools for AutoML, such as Auto-WEKA, TPOT, and auto-sklearn, mainly deal with single-label classification and regression, there is very little work on other types of machine learning tasks. In particular, there is almost no work on automating the engineering of machine learning applications for multi-label classification. This paper makes two contributions. First, it discusses the usefulness and feasibility of an AutoML approach for multi-label classification. Second, we show how the scope of ML-Plan, an AutoML-tool for multi-class classification, can be extended towards multi-label classification using MEKA, which is a multi-label extension of the well-known Java library WEKA. The resulting approach recursively refines MEKA's multi-label classifiers, which sometimes nest another multi-label classifier, up to the selection of a single-label base learner provided by WEKA. In our evaluation, we find that the proposed approach yields superb results and performs significantly better than a set of baselines.

==> tables/datasets.tex <==
\resizebox{\columnwidth}{!}{
\begin{tabular}{llll}
\hline
Dataset & \# Inst. & \#Feat. & \#Labels\\
\hline
arts & & & \\
bibtex & 7395 & 1836 & 159 \\
bookmarks & 87856 & 2150 & 208 \\
birds & 645 & 260 & 19 \\
Business1 & & \\
Computers1 & & \\
Education1 & & \\
Enron & 1705 & 1001 & 53 \\
Entertainment1 & & \\
flags & 194 & 19 & 7 \\
Health1 & & \\
LangLog & & \\
MEDC & & \\
mediamill & 43907 & 120 & 101 \\
musicout & & & \\
protein & & \\
Recreation1 & & \\
Reference & & \\
scene & 2407 & 294 & 6 \\
Science1 & & \\
Social1 & & \\
Society1 & & \\
tmc & 28596 & 32786$\pm$7990 & 31$\pm$6 \\
yeast & 2417 & 103 & 14\\
\hline
\end{tabular}}

==> tables/results_exact.tex <==
\small
\bgroup
\def\arraystretch{1} % row height: 1 is the default
\setlength\tabcolsep{2.5pt} % col width: 6 is the default
\resizebox{\textwidth}{!}{
\begin{tabular}{l||r|r|r|r|r|r}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{1}{c|}{1m\TBstrut} & \multicolumn{2}{c|}{1h\TBstrut}  & \multicolumn{2}{c|}{12h\TBstrut}\\
& Auto-MEKA & Auto-MEKA & BR-Auto-WEKA & Auto-MEKA & BR-Auto-WEKA\\\hline
{\sc Arts} & 0.1735$\pm$0.0091 (12) & 0.3998$\pm$0.0699 (9) &  & 0.4261$\pm$0.0145 (4) & \\
{\sc Bibtex} & 0.0603$\pm$0.0162 (9) & 0.1674$\pm$0.0065 (10) &  & 0.1625$\pm$0.0213 (4) & \\
{\sc Birds} & 0.0792$\pm$0.0190 (9) & 0.0937$\pm$0.0231 (8) &  & 0.1047$\pm$0.0113 (4) & 0.1085$\pm$3.0E-4 (3)\\
{\sc Bookmarks} & 0.1010$\pm$0.0333 (6) & 0.1906$\pm$0.0138 (9) &  & 0.1837$\pm$0.0000 (1) & \\
{\sc Business} & 0.5317$\pm$0.0119 (9) & 0.5359$\pm$0.0392 (9) &  & 0.6024$\pm$0.0000 (1) & \\
{\sc Computers} & 0.3293$\pm$0.0067 (8) & 0.3625$\pm$0.0611 (10) &  & 0.5375$\pm$0.0065 (3) & \\
{\sc Education} & 0.2227$\pm$0.0074 (8) & 0.3891$\pm$0.0866 (10) &  & 0.4315$\pm$0.0070 (3) & \\
{\sc Enron} & 0.0745$\pm$0.0333 (7) & 0.1287$\pm$0.0119 (10) &  & \textbf{0.1401}$\pm$0.0082 (4) & 0.0777$\pm$0.0551 (3)\\
{\sc Entertainment} & 0.2201$\pm$0.0177 (9) & 0.3371$\pm$0.1457 (8) &  & 0.5879$\pm$0.0031 (4) & \\
{\sc Flags} & 0.1239$\pm$0.0527 (10) & 0.0939$\pm$0.0438 (9) & 0.0819$\pm$0.0501 (8) & 0.1150$\pm$0.0665 (3) & 0.0863$\pm$0.0372 (3)\\
{\sc Health} & 0.3113$\pm$0.0096 (8) & 0.4877$\pm$0.1392 (8) &  & 0.5957$\pm$0.0048 (3) & \\
{\sc LangLog} & 0.2077$\pm$0.0306 (8) & 0.2999$\pm$0.0264 (9) &  & 0.2936$\pm$0.0242 (3) & \\
{\sc MEDC} & 0.6642$\pm$0.0202 (9) & 0.6765$\pm$0.0179 (9) &  & 0.6519$\pm$0.0169 (3) & 0.6332$\pm$0.0051 (2)\\
{\sc Mediamill} & 0.0541$\pm$0.0014 (8) & 0.1638$\pm$0.0793 (8) &  & 0.2293$\pm$0.0040 (3) & \\
{\sc Musicout} & 0.3041$\pm$0.0436 (10) & \textbf{0.2935}$\pm$0.0452 (10) & 0.2231$\pm$0.0317 (10) & 0.3183$\pm$0.0076 (2) & 0.2630$\pm$0.0235 (4)\\
{\sc Protein} & 0.9692$\pm$0.0108 (8) & 0.9688$\pm$0.0131 (10) & 0.5277$\pm$0.0000 (1) & \textbf{0.9715}$\pm$0.0048 (3) & 0.8504$\pm$0.1486 (4)\\
{\sc Recreation} & 0.1674$\pm$0.0275 (8) & 0.2879$\pm$0.1650 (10) &  & 0.5459$\pm$0.0072 (4) & \\
{\sc Reference} & 0.3824$\pm$0.0080 (10) & 0.4811$\pm$0.0966 (10) &  & 0.5717$\pm$0.0096 (3) & \\
{\sc Scene} & 0.4090$\pm$0.1602 (8) & \textbf{0.6928}$\pm$0.0409 (8) & 0.5435$\pm$0.0199 (9) & \textbf{0.6951}$\pm$0.0663 (4) & 0.5551$\pm$0.0295 (4)\\
{\sc Science} & 0.1872$\pm$0.0103 (9) & 0.3977$\pm$0.1361 (10) &  & 0.4899$\pm$0.0074 (3) & \\
{\sc Social} & 0.3629$\pm$0.0351 (8) & 0.4157$\pm$0.0980 (10) &  & 0.6101$\pm$0.0093 (2) & \\
{\sc Society} & 0.2759$\pm$0.0132 (10) & 0.3067$\pm$0.0542 (10) &  & 0.3641$\pm$0.0783 (3) & \\
{\sc Tmc} & 0.0869$\pm$0.0010 (3) & 0.0827$\pm$0.0151 (8) &  &  & \\
{\sc Yeast} & 0.1115$\pm$0.0456 (7) & \textbf{0.1931}$\pm$0.0107 (9) & 0.0832$\pm$0.0569 (6) & 0.1980$\pm$0.0088 (3) & 0.0697$\pm$0.0586 (2)\\
    \end{tabular}}
    \caption{Exact (to be maximized).}
    \egroup


==> tables/results_hamming.tex <==
\small
\bgroup
\def\arraystretch{1} % row height: 1 is the default
\setlength\tabcolsep{2.5pt} % col width: 6 is the default
\resizebox{\textwidth}{!}{
\begin{tabular}{l||r|r|r|r|r|r}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{1}{c|}{1m\TBstrut} & \multicolumn{2}{c|}{1h\TBstrut}  & \multicolumn{2}{c|}{12h\TBstrut}\\
& Auto-MEKA & Auto-MEKA & BR-Auto-WEKA & Auto-MEKA & BR-Auto-WEKA\\\hline
arts&$0.0831\pm0.0014$&$0.0548\pm0.0014$&-&-&-\\
bibtex&$0.0212\pm0.0011$&$0.0167\pm4.0E-4$&-&-&-\\
bookmarks&$0.0141\pm0.0011$&$0.0136\pm0.0015$&-&-&-\\
birds: -C -21&$0.0915\pm0.0052$&$0.0851\pm0.0086$&-&-&-\\
Business1: -C -30&$0.029\pm7.0E-4$&$0.0282\pm0.0024$&-&-&-\\
Computers1: -C -33&$0.0446\pm9.0E-4$&$0.0419\pm0.0051$&-&-&-\\
Education1: -C -33&$0.0554\pm6.0E-4$&$0.0376\pm5.0E-4$&-&-&-\\
Enron: -C 53 -split-number 1135&$0.0555\pm0.003$&$0.0549\pm0.0046$&-&-&-\\
Entertainment1: -C -21&$0.0894\pm0.0074$&$0.0818\pm0.0174$&-&-&-\\
flags&$0.2191\pm0.0166$&$0.2095\pm0.012$&$0.204\pm0.0212$&-&-\\
Health1: -C -32&$0.0507\pm8.0E-4$&$0.0331\pm0.0101$&-&-&-\\
LangLog: -C 75&$0.0238\pm0.0027$&$0.0207\pm7.0E-4$&-&-&-\\
MEDC: -C -45&$0.0111\pm0.0011$&$0.0111\pm9.0E-4$&-&-&-\\
mediamill-train-exp1: -C -101&$0.0417\pm4.0E-4$&$0.0325\pm8.0E-4$&-&-&-\\
musicout: -C -6&$0.2107\pm0.0187$&$0.2234\pm0.0224$&$0.2191\pm0.0101$&-&-\\
protein: -C -27&$0.0013\pm5.0E-4$&$0.0013\pm3.0E-4$&$0.0174\pm0.0$&-&-\\
Recreation1: -C -22&$0.0899\pm0.0024$&$0.0784\pm0.0229$&-&-&-\\
Reference1: -C -33&$0.0376\pm0.001$&$0.0311\pm0.006$&-&-&-\\
scene: -C -6&$0.1666\pm0.0455$&$0.0912\pm0.0076$&$0.0998\pm0.0046$&-&-\\
Science1: -C -40&$0.0491\pm6.0E-4$&$0.0302\pm4.0E-4$&-&-&-\\
Social1: -C -39&$0.0355\pm0.0021$&$0.0358\pm9.0E-4$&-&-&-\\
Society1: -C -27&$0.0635\pm0.003$&$0.0607\pm0.0043$&-&-&-\\
tmc: -C -22&$0.1164\pm4.0E-4$&$0.0996\pm0.0075$&-&-&-\\
yeast: -C -14&$0.2355\pm0.0129$&$0.2055\pm0.0028$&$0.2202\pm0.0183$&-&-\\
    \end{tabular}}
    \caption{Hamming (to be minimized).} 
    \egroup


==> tables/results_jaccard.tex <==
\small
\bgroup
\def\arraystretch{1} % row height: 1 is the default
\setlength\tabcolsep{2.5pt} % col width: 6 is the default
\resizebox{\textwidth}{!}{
\begin{tabular}{l||r|r|r|r|r|r}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{1}{c|}{1m\TBstrut} & \multicolumn{2}{c|}{1h\TBstrut}  & \multicolumn{2}{c|}{12h\TBstrut}\\
& Auto-MEKA & Auto-MEKA & BR-Auto-WEKA & Auto-MEKA & BR-Auto-WEKA\\\hline
arts&$0.2091\pm0.0126$&$0.5003\pm0.0125$&-&-&-\\
bibtex&$0.089\pm0.023$&$0.2827\pm0.0042$&-&-&-\\
bookmarks&$0.1049\pm0.0348$&$0.2077\pm0.0129$&-&-&-\\
birds: -C -21&$1.0\pm0.0$&$1.0\pm0.0$&-&-&-\\
Business1: -C -30&$0.675\pm0.0082$&$0.6885\pm0.0328$&-&-&-\\
Computers1: -C -33&$0.4081\pm0.0064$&$0.4536\pm0.0805$&-&-&-\\
Education1: -C -33&$0.2613\pm0.0061$&$0.5044\pm0.0048$&-&-&-\\
Enron: -C 53 -split-number 1135&$0.3561\pm0.0344$&$0.4291\pm0.0123$&-&-&-\\
Entertainment1: -C -21&$0.2538\pm0.0176$&$0.3497\pm0.1256$&-&-&-\\
flags&$0.5177\pm0.0319$&$0.5436\pm0.0208$&$0.5328\pm0.0317$&-&-\\
Health1: -C -32&$0.3951\pm0.0099$&$0.6266\pm0.1198$&-&-&-\\
LangLog: -C 75&$1.0\pm0.0$&$1.0\pm0.0$&-&-&-\\
MEDC: -C -45&$0.7483\pm0.0156$&$0.7623\pm0.0127$&-&-&-\\
mediamill-train-exp1: -C -101&$0.4092\pm0.2233$&$1.0\pm0.0$&-&-&-\\
musicout: -C -6&$0.5734\pm0.0313$&$0.5606\pm0.0355$&$0.4941\pm0.0249$&-&-\\
protein: -C -27&$0.985\pm0.0054$&$0.9826\pm0.0055$&$0.5725\pm0.0$&-&-\\
Recreation1: -C -22&$0.1971\pm0.0303$&$0.3438\pm0.1849$&-&-&-\\
Reference1: -C -33&$0.4257\pm0.0074$&$0.5257\pm0.0985$&-&-&-\\
scene: -C -6&$0.5689\pm0.0494$&$0.7371\pm0.0152$&$0.6079\pm0.0201$&-&-\\
Science1: -C -40&$0.2111\pm0.0109$&$0.5405\pm0.0083$&-&-&-\\
Social1: -C -39&$0.4033\pm0.0351$&$0.4121\pm0.018$&-&-&-\\
Society1: -C -27&$0.3624\pm0.0148$&$0.3888\pm0.0549$&-&-&-\\
tmc: -C -22&$0.17\pm0.003$&$0.2785\pm0.0128$&-&-&-\\
yeast: -C -14&$0.49\pm0.0143$&$0.541\pm0.004$&$0.4925\pm0.0215$&-&-\\
    \end{tabular}}
    \caption{Jaccard (to be maximized).} 
    \egroup


==> tables/results_rank.tex <==
\small
\bgroup
\def\arraystretch{1} % row height: 1 is the default
\setlength\tabcolsep{2.5pt} % col width: 6 is the default
\resizebox{\textwidth}{!}{
\begin{tabular}{l||r|r|r|r|r|r}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{1}{c|}{1m\TBstrut} & \multicolumn{2}{c|}{1h\TBstrut}  & \multicolumn{2}{c|}{12h\TBstrut}\\
& Auto-MEKA & Auto-MEKA & BR-Auto-WEKA & Auto-MEKA & BR-Auto-WEKA\\\hline
arts&$0.0318\pm0.0015$&$0.0188\pm8.0E-4$&-&-&-\\
bibtex&$0.0071\pm0.001$&$0.0049\pm4.0E-4$&-&-&-\\
bookmarks&$0.0049\pm0.0012$&$0.0051\pm0.0014$&-&-&-\\
birds: -C -21&$0.0\pm0.0$&$0.0\pm0.0$&-&-&-\\
Business1: -C -30&$0.0092\pm0.0123$&$0.008\pm0.0078$&-&-&-\\
Computers1: -C -33&$0.0248\pm0.0259$&$0.014\pm0.0019$&-&-&-\\
Education1: -C -33&$0.0216\pm2.0E-4$&$0.0258\pm0.0197$&-&-&-\\
Enron: -C 53 -split-number 1135&$0.0455\pm0.0557$&$0.0138\pm0.0024$&-&-&-\\
Entertainment1: -C -21&$0.0376\pm0.0041$&$0.0343\pm0.0083$&-&-&-\\
flags&$0.0858\pm0.0413$&$0.1136\pm0.0444$&$0.1635\pm0.0213$&-&-\\
Health1: -C -32&$0.0162\pm4.0E-4$&$0.0232\pm0.0111$&-&-&-\\
LangLog: -C 75&$0.0\pm0.0$&$0.0\pm0.0$&-&-&-\\
MEDC: -C -45&$0.009\pm0.0118$&$0.0061\pm0.007$&-&-&-\\
mediamill-train-exp1: -C -101&$0.0\pm0.0$&$0.0\pm0.0$&-&-&-\\
musicout: -C -6&$0.1023\pm0.0325$&$0.1098\pm0.0196$&$0.1865\pm0.0213$&-&-\\
protein: -C -27&$7.0E-4\pm0.0012$&$0.0\pm1.0E-4$&$0.0039\pm0.0$&-&-\\
Recreation1: -C -22&$0.0384\pm8.0E-4$&$0.0573\pm0.0201$&-&-&-\\
Reference1: -C -33&$0.0166\pm4.0E-4$&$0.0202\pm0.0144$&-&-&-\\
scene: -C -6&$0.0907\pm0.0262$&$0.0582\pm0.0199$&$0.0705\pm0.0099$&-&-\\
Science1: -C -40&$0.0197\pm3.0E-4$&$0.0227\pm0.0256$&-&-&-\\
Social1: -C -39&$0.0147\pm0.001$&$0.0151\pm4.0E-4$&-&-&-\\
Society1: -C -27&$0.0205\pm0.0017$&$0.0192\pm0.0017$&-&-&-\\
tmc: -C -22&$0.0353\pm3.0E-4$&$0.1053\pm0.0616$&-&-&-\\
yeast: -C -14&$0.1185\pm0.0309$&$0.0911\pm0.0038$&$0.1757\pm0.0033$&-&-\\
    \end{tabular}}
    \caption{Rank (to be minimized).} 
    \egroup


==> tables/usedClassifiers.tex <==
\begin{tabular}{lll}
\hline
Classifier & Times Used \\
\hline
BCC & \\
BR & \\
CC & \\
CT & \\
CDN & \\
CDT & \\
MCC & \\
PCC & \\
PMCC & \\

MajorityLabelset & \\
LC & \\
PS & \\
PSt & \\
SCC & \\
RAkEL & \\
RAkELd & \\
SERAkELd & \\
HASEL & \\
MULAN & \\
FW & \\
RT & \\
EM & \\
\hline
\end{tabular}



==> tables/usedWekaClassifiers.tex <==
\begin{tabular}{lll}
\hline
Classifier & Times Used \\
\hline
BayesNet & \\
NaiveBayes & \\
NaiveBayesMultinomial & \\
GaussianProcesses & \\
LinearRegression & \\
Logistic & \\
MultilayerPerceptron & \\
SGD & \\
SimpleLinearRegression & \\
SimpleLogistic & \\
SMO & \\
SMOreg & \\
VotedPerceptron & \\
IBk & \\
KStar & \\
DecisionTable & \\
JRip & \\
M5Rules & \\
OneR & \\
PART & \\
ZeroR & \\
DecisionStump & \\
J48 & \\
LMT & \\
M5P & \\
RandomForest & \\
RandomTree & \\
REPTree & \\
LWL & \\
AdditiveRegression & \\
AdaBoostM1 & \\
AttributeSelectedClassifier & \\
Bagging & \\
ClassificationViaRegression & \\
LogitBoost & \\
MultiClassClassifier & \\
RandomCommittee & \\
RandomSubSpace & \\
Vote & \\
Stacking & \\
MultiBoostAB & \\
\hline
\end{tabular}
